Applying machine learning to determine impact parameter in nuclear physics experiments

Machine Learning (ML) algorithms have been demonstrated to be capable of predicting impact parameter in heavy-ion collisions from transport model simulation events with perfect detector response. We extend the scope of ML application to experimental data by incorporating realistic detector response of the S$\pi$RIT Time Projection Chamber into the heavy-ion simulation events generated from the UrQMD model to resemble experimental data. At 3 fm, the predicted impact parameter is 2.8 fm if simulation events with perfect detector is used for training and testing; 2.4 fm if detector response is included in the training and testing, and 5.8 fm if ML algorithms trained with perfect detector is applied to testing data that has included detector response. The last result is not acceptable illustrating the importance of including the detector response in developing the ML training algorithm. We also test the model dependence by applying the algorithms trained on UrQMD model to simulated events from four different transport models as well as using different input parameters on UrQMD model. Using data from Sn+Sn collisions at E/A=270 MeV, the ML determined impact parameters agree well with the experimentally determined impact parameter using multiplicities, except in the very central and very peripheral regions. ML selects central collision events better and allows impact parameters determination beyond the sharp cutoff limit imposed by experimental methods.

==> ML_Impact_parameter (Copy)/authors.tex <==
% repeat the \author .. \affiliation  etc. as needed
% \email, \thanks, \homepage, \altaffiliation all apply to the current
% author. Explanatory text should go in the []'s, actual e-mail
% address or url should go in the {}'s for \email and \homepage.
% Please use the appropriate macro foreach each type of information

% \affiliation command applies to all authors since the last
% \affiliation command. The \affiliation command should follow the
% other information
% \affiliation can be followed by \email, \homepage, \thanks as well.

\author{C.Y.~Tsang}%~(\CJKfamily{bsmi}{曾}}
\affiliation{National Superconducting Cyclotron Laboratory, Michigan State University, East Lansing, Michigan 48824, USA}
\affiliation{Department of Physics, Michigan State University, East Lansing, Michigan 48824, USA}

\author{Yongjia Wang}
\affiliation{School of Science, Huzhou University, Huzhou 313000, China}

\author{M.B.~Tsang}%~(\CJKfamily{bsmi}{曾敏兒})}
%\altaffiliation{Corresponding author}
%\email{tsang@nscl.msu.edu}
\affiliation{National Superconducting Cyclotron Laboratory, Michigan State University, East Lansing, Michigan 48824, USA}
\affiliation{Department of Physics, Michigan State University, East Lansing, Michigan 48824, USA}

\author{J.~Estee}
%\altaffiliation{Corresponding author}
%\email{esteejus@mit.edu}
\affiliation{National Superconducting Cyclotron Laboratory, Michigan State University, East Lansing, Michigan 48824, USA}
\affiliation{Department of Physics, Michigan State University, East Lansing, Michigan 48824, USA}

\author{T.~Isobe}%~(\CJKfamily{min}{磯部忠昭})}
%\altaffiliation{Corresponding author}
%\email{isobe@riken.jp}
\affiliation{RIKEN Nishina Center, Hirosawa 2-1, Wako, Saitama 351-0198, Japan}

\author{M.~Kaneko}%~(\CJKfamily{min}{金子雅紀})}
\affiliation{RIKEN Nishina Center, Hirosawa 2-1, Wako, Saitama 351-0198, Japan}
\affiliation{Department of Physics, Kyoto University, Kita-shirakawa, Kyoto 606-8502, Japan}

\author{M.~Kurata-Nishimura}%~(\CJKfamily{min}{倉田-西村美月})}
\affiliation{RIKEN Nishina Center, Hirosawa 2-1, Wako, Saitama 351-0198, Japan}

\author{J.W.~Lee}%~(\CJKfamily{mj}{이정우})}
\affiliation{Department of Physics, Korea University, Seoul 02841, Republic of Korea}

\author{Fupeng Li}
\affiliation{School of Science, Huzhou University, Huzhou 313000, China}
\affiliation{College of Science, Zhejiang University of Technology, Hangzhou 310014, China}
\author{Qingfeng Li}
\affiliation{School of Science, Huzhou University, Huzhou 313000, China}
\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou 730000, China}

\author{W.G.~Lynch}%~(\CJKfamily{bsmi}{連致標})}
%\altaffiliation{Corresponding author}
%\email{lynch@nscl.msu.edu}
\affiliation{National Superconducting Cyclotron Laboratory, Michigan State University, East Lansing, Michigan 48824, USA}
\affiliation{Department of Physics, Michigan State University, East Lansing, Michigan 48824, USA}



\author{T.~Murakami}%~(\CJKfamily{min}{村上哲也})}
%\altaffiliation{Corresponding author}
%\email{murakami.tetsuya.3e@kyoto-u.ac.jp}
\affiliation{RIKEN Nishina Center, Hirosawa 2-1, Wako, Saitama 351-0198, Japan}
\affiliation{Department of Physics, Kyoto University, Kita-shirakawa, Kyoto 606-8502, Japan}

\author{R.~Wang}%~(\CJKfamily{gbsn}{王})}
\affiliation{National Superconducting Cyclotron Laboratory, Michigan State University, East Lansing, Michigan 48824, USA}



\author{Dan~Cozma}
\affiliation{IFIN-HH, Reactorului 30, 077125 M\v{a}gurele-Bucharest, Romania}

\author{Rohit~Kumar}
\affiliation{National Superconducting Cyclotron Laboratory, Michigan State University, East Lansing, Michigan 48824, USA}

\author{Akira~Ono}
\affiliation{Department of Physics, Tohoku University, Sendai 980-8578, Japan}

\author{Ying-Xun~Zhang}
\affiliation{China Institute of Atomic Energy, Beijing 102413, China}




%\author{P.~Danielewicz}
%%\author{D.~Oliinychenko}
%\author{H.~Elfnerg}
%\author{N.~Ikeno}
%\author{C.M.~Ko}
%\author{J. Moh}
%\author{A.~Ono}
%\author{J.~Su}
%\author{Yong Jia Wang}
%\author{H.~Wolter}
%\author{Zhen Zhang}
%\author{Ying-Xun Zhang}
%\noaffiliation
%\collaboration{TMEP collaboration}
%\noaffiliation




%Collaboration name if desired (requires use of superscriptaddress
%option in \documentclass). \noaffiliation is required (may also be
%used with the \author command).
%\collaboration can be followed by \email, \homepage, \thanks as well.
%\collaboration{}
%\noaffiliation
